Learning Certified Individually Fair Representations

Fair representation learning provides an effective way of enforcing fairness constraints without compromising utility for downstream users. A desirable family of such fairness constraints, each requiring similar treatment for similar individuals, is known as individual fairness. In this work, we introduce the first method that enables data consumers to obtain certificates of individual fairness for existing and new data points. The key idea is to map similar individuals to close latent representations and leverage this latent proximity to certify individual fairness. That is, our method enables the data producer to learn and certify a representation where for a data point all similar individuals are at $\ell_\infty$-distance at most $\epsilon$, thus allowing data consumers to certify individual fairness by proving $\epsilon$-robustness of their classifier. Our experimental evaluation on five real-world datasets and several fairness constraints demonstrates the expressivity and scalability of our approach.

==> figures/vary_noise.tex <==
% This file was created by matplotlib2tikz v0.7.4.
\pgfplotsset{every axis/.append style={
    %label style={font=\LARGE},
    %tick label style={font=\LARGE},
    %legend style={font=\LARGE}
}}
\begin{tikzpicture}

    \definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
    \definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
    \definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}

    \begin{axis}[
        grid style={draw=white},
        legend cell align={left},
        legend style={draw=none, fill=none, at={(0.4,0.1)}, anchor=south east},
        ymajorgrids=true,
        tick align=outside,
        tick pos=left,
        xlabel={Noise level $\alpha$},
        xmin=-0.05, xmax=0.55,
        axis x line=bottom,
        axis y line=left,
        minor tick num=0,
        ymin=-5, ymax=110,
        ytick style={color=black},
        %ytick={-20,0,20,40,60,80,100,120},
        %yticklabels={-20,0,20,40,60,80,100,120},
        axis background/.style={fill=gray!14}
    ]
        \addplot [semithick, color0, mark=triangle*, mark size=3, mark options={solid}]
        table {%
        0.0 82.2
        0.1 0
        0.2 81.4
        0.3 81.3
        0.4 81.1
        0.5 81.1
        };
        \addlegendentry{Accuracy}
        \addplot [semithick, color1, mark=triangle*, mark size=3, mark options={solid}]
        table {%
        0.0 99.5
        0.1 0
        0.2 97.4
        0.3 97.9
        0.4 97.6
        0.5 97.7
        };
        \addlegendentry{Certified}
    \end{axis}

\end{tikzpicture}


==> headers/lqa/colors.tex <==
% Description: This file contains a few useful colors.
%
% Usage: You may need to comment out the usepackage command below, if they
% conflict with your conference template


%%%%%%%%%
% SETUP %
%%%%%%%%%
% import relevant packages

\usepackage[usenames, dvipsnames]{color} % for textcolor
\usepackage{xcolor} % for definecolor


%%%%%%%%%%%%%%%%%%%%%%
%  MATPLOTLIB COLORS %
%%%%%%%%%%%%%%%%%%%%%%


% blue
\definecolor{my-full-blue}{HTML}{1F77B4}
%\definecolor{blue}{RGB}{31,119,180} 

% orange
\definecolor{my-full-orange}{HTML}{FF7F0E}
%\definecolor{orange}{RGB}{255,127,14}

% green
\definecolor{my-full-green}{HTML}{2CA02C}
%\definecolor{green}{RGB}{44,160,44}

% red
\definecolor{my-full-red}{HTML}{d62728}
%\definecolor{red}{RGB}{214,39,40}

% purple
\definecolor{my-full-purple}{HTML}{9467bd}
%\definecolor{purple}{RGB}{148,103,189}

% lighter shades
\colorlet{my-blue}{my-full-blue!30}
\colorlet{my-orange}{my-full-orange!30}
\colorlet{my-green}{my-full-green!30}
\colorlet{my-red}{my-full-red!30}
\colorlet{my-purple}{my-full-purple!30}


%%%%%%%%%%%%%%%%%%%%%%
%  PROJECT-SPECIFIC  %
%%%%%%%%%%%%%%%%%%%%%%
% add project-specific colors here

==> headers/lqa/subfigures.tex <==
% Description: This file introduces a subfigure which correctly aligns
% captions
%
% Usage:
% - \input{headers/lqa/subfigures}
% - You may need to comment out the usepackage command below in case of
%   conflicts

% EXAMPLE USAGE:
%
% \begin{figure}
% 	\centering
% 	\mysubfigure[0.49\linewidth]{
% 		\centering
% 		Content of subfigure 1
% 	}{Caption of subfigure\label{fig:subfig1}}
% 	\mysubfigure[0.49\linewidth]{
% 		\centering
% 		Content of subfigure 2
% 	}{Caption of subfigure\label{fig:subfig2}}
% 	\caption{An example of subfigures.}
% 	\label{fig:subfigures}
% \end{figure}

%%%%%%%%%%%%%%
% USEPACKAGE %
%%%%%%%%%%%%%%
\usepackage{subcaption}

%%%%%%%%%%%
% COMMAND %
%%%%%%%%%%%

\newcommand{\mysubfigure}[3][\linewidth]{\subcaptionbox{#3}[#1]{
	\begin{minipage}{#1}
		% uses minipage to prevent unexpected interactions,
		% e.g., for align
		#2
	\end{minipage}
}}

